Maximal distance minimizers for a rectangle

\emph{A maximal distance minimizer} for a given compact set $M \subset \mathbb{R}^2$ and some given $r > 0$ is a set having the minimal length (one-dimensional Hausdorff measure) over the class of closed connected sets $\Sigma \subset \mathbb{R}^2$ satisfying the inequality \[ \max_{y\in M} dist (y, \Sigma) \leq r. \] This paper deals with the set of maximal distance minimizers for a rectangle $M$ and small enough $r$.

==> pictures/Presentation90.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=1cm,y=1cm, scale = 1]
    
        \coordinate (V) at (1.4511769417267553,1.2941342560758087);
        \coordinate (W1) at (2.8223786956631924,0.9942091784463614);
        \coordinate (W2) at (0.9881455681973705,2.748339302798502);
    
        \draw [shift={(2.7149165651566225,0)},] (0:0.2558385377085195) arc (0:83.83096092621358:0.2558385377085195);
        
        \draw [shift={(W1)},] (0:0.22) arc (0:83.8309609262136:0.22);
        \draw [shift={(W1)},] (83.8309609262136:0.2558385377085195) arc (83.8309609262136:167.66192185242716:0.2558385377085195);
        
        
        \draw [shift={(0,2.5948194798051945)},] (8.830960926213633:0.2558385377085195) arc (8.830960926213633:90:0.2558385377085195);
        \draw [shift={(0,2.5948194798051945)},] (8.830960926213633:0.20040685453834028) arc (8.830960926213633:90:0.20040685453834028);
        \draw [shift={(W2)},] (8.83096092621364:0.2558385377085195) arc (8.83096092621364:90:0.2558385377085195);
        \draw [shift={(W2)},] (8.83096092621364:0.20040685453834028) arc (8.83096092621364:90:0.20040685453834028);
        \draw [shift={(W2)},] (-72.33807814757273:0.21319878142376622) arc (-72.33807814757273:8.830960926213644:0.21319878142376622);
        \draw [shift={(W2)},] (-72.33807814757273:0.157767098253587) arc (-72.33807814757273:8.830960926213644:0.157767098253587);
        
        \draw [very thick] (0,4.5)-- (0,0);
        \draw [very thick] (5,0)-- (0,0);
        \draw [] (1,0) arc (0 : 90 : 1);
        \draw [] (0,1.5948194798051945) arc (-90 : 90 : 1);
        \draw [] (3.7149165651566225,0) arc (0 : 180 : 1);
        \draw [,dashed] (0.5257398542969663,0.8506454053269227)-- (0,0)
            node[pos=0.4,below right]{$r$};
        \draw [thick, blue] (0.9881455681973705,4.043597731705948)-- (W2);
        \draw [thick, blue] (W2)-- (V);
        \draw [thick, blue] (V)-- (W1);
        \draw [thick, blue] (W1)-- (4.430166711325904,0.9942091784463614);
        \draw [,dashed] (0,2.5948194798051945)-- (W2)
            node[pos=0.5, below]{$r$};
        \draw [,dashed] (W2)-- (1.560382488301416,2.837242915294451);
        \draw [,dashed] (2.7149165651566225,0)-- (W1)
            node[pos=0.5, left]{$r$};
        \draw [,dashed] (W1)-- (2.891073104860997,1.629750385478656);
        \draw [] (4.430166711325904,1)-- (4.430166711325904,0);
        \draw [] (1,4.043597731705948)-- (0,4.043597731705948);
        \draw [thick, blue,dashed] (1.2367685238557085,1.0588168446924053)-- (1.0328898481033684,0.8350560302118302);
        \draw [thick, blue] (1.2367685238557085,1.0588168446924053)-- (V);
        
        \draw [decorate , decoration={brace, mirror, amplitude=3pt},      
            xshift=0pt,yshift=-4pt]
        (0, 0) -- (2.7149165651566225,0) node [midway,yshift=-0.5cm] {$x$};
        \draw [decorate , decoration={brace, amplitude=3pt},      
            xshift=-4pt,yshift=0pt]
        (0, 0) -- (0,2.5948194798051945) node [midway,xshift=-0.5cm] {$y$};
        
        \def\nodesize{0.03}
        
        \fill [] (0,0) circle (\nodesize)
            node[below left]{$A_1$};
        \fill [] (0,4.5)
            node[above]{$A_3$};
        \fill [] (5,0)
            node[right]{$A_2$};
            
        \fill [blue] (W1) circle (\nodesize)
            node[black, below left]{$W_1$};
        \draw[shift={(W1)}] (0.15, 0.05)
            node[above right]{\large $\alpha$};
        \fill [] (2.7149165651566225,0) circle (\nodesize)
            node[below right]{$y(W_1)$};
            
            
        \fill [blue] (W2) circle (\nodesize)
            node[black, above left]{$W_2$};
        \draw[shift={(W2)}] (0.1, 0.15)
            node[above right]{\large $\beta$};
        \fill [] (0,2.5948194798051945) circle (\nodesize)
            node[above left]{$y(W_2)$};
            
            
        \fill [blue] (V) circle (\nodesize)
            node[black, above right]{$V$}
            node[black, left]{$120^\circ$};
        \draw[shift={(V)}] (0.1, -0.05) 
            node[below]{$120^\circ$};
            
        \fill [blue] (0.9881455681973705,4.043597731705948) circle (\nodesize)
            node[black, above]{$Z_2$};
        \fill [blue] (4.430166711325904,0.9942091784463614) circle (\nodesize)
            node[black, right]{$Z_2$};
        \fill [] (0,4.043597731705948) circle (\nodesize)
            node[left]{$C_{12}$};
        \fill [] (4.430166711325904,0) circle (\nodesize)
            node[below]{$C_{11}$};
        \fill [] (1.1,4.043597731705948)
            node[right]{$D_{12}$};
        \fill [] (4.430166711325904,1.1) 
            node[above]{$D_{11}$};;
    \end{tikzpicture}
   % \caption{Пересечение $\mathcal{C}$ с окрестностью угла}
    \label{minimizer90}
\end{figure}

==> pictures/PresentationStadion.tex <==
\begin{figure}[h]
    \centering
 

\begin{tikzpicture}[scale=1.1]

\foreach \y in {0, 3.51389977019889} {
    \draw[very thick, loosely dotted] 
        (-1, \y) -- (0, \y);
    \draw[very thick]
        (0, \y) -- (3.66, \y);
    \draw[very thick, loosely dotted] 
        (3.66, \y) -- (4.66, \y);
}
\draw[very thick] (-1, 0) arc (270:90:1.757);
\draw[very thick] (4.66, 0) arc (-90:90:1.757);


%\draw[thin, dashed] (0.2614137092297641 + 1, 0.0) arc (0:180:1);
%\draw[thin, dashed] (0.7842411276892922 + 1, 0.0) arc (0:180:1);
%\draw[thin, dashed] (1.3070685461488205 + 1, 0.0) arc (0:180:1);
\draw[thin, dashed] (1.8298959646083486 + 1, 0.0) arc (0:180:1);
%\draw[thin, dashed] (2.3527233830678767 + 1, 0.0) arc (0:180:1);
%\draw[thin, dashed] (2.875550801527405 + 1, 0.0) arc (0:180:1);
%\draw[thin, dashed] (3.398378219986933 + 1, 0.0) arc (0:180:1);
%\draw[thin, dashed] (1.8298959646083486 + 1, 3.75) arc (0:-180:1);


\draw[blue, thick] 
(0.0, 0.9652268503449002) -- 
(1.5684822553785844, 0.9652268503449002) --
(1.8298959646083486, 1.11615412573856) --
(2.0913096738381127, 0.9652268503449002) -- 
(3.659791929216697, 0.9652268503449002);

\node[blue] at (1.61,1.8) {$\Sigma_0$};

\draw[dashed] (0.0, 0.0) -- (0.0, 3.51389977019889);
\draw[dashed] (3.659791929216697, 0.0) -- (3.659791929216697, 3.51389977019889);

\fill[blue] (0.0, 0.9652268503449002) 
    circle (1.5pt) node[black, below right] {$A$};
\fill[blue] (3.659791929216697, 0.9652268503449002) 
    circle (1.5pt) node[black, below left] {$B$};

\draw[blue, thick] 
(1.8298959646083486, 1.11615412573856) -- 
(1.8298959646083486, 2.58208251632886);

\draw[thin, dashed] (1, 3.51389977019889) arc (0:-90:1);
\draw[thin, dashed] (2.66, 3.51389977019889) arc (180:270:1);

\draw[blue, thick]
(1.8298959646083486, 2.58208251632886) -- 
(0.9149479823041743, 3.11032798020668);

\draw[blue, thick] 
(1.8298959646083486, 2.58208251632886) -- 
(2.744843946912523, 3.11032798020668);



\end{tikzpicture}

\caption{A horseshoe is not optimal for long enough stadium if $R < 1.75r$.}
%КАЖЕТСЯ ЛИБО ЛОНГЭНАФ ЛИБО НЕРАВЕНСТВО. И НАВЕРНОЕ НЕ ДЛИННЫЙ А УЗКИЙ?
    \label{stadion}
\end{figure}

==> ����������� (1)/pictures/Presentation90.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=1cm,y=1cm, scale = 1]
    
        \coordinate (V) at (1.4511769417267553,1.2941342560758087);
        \coordinate (W1) at (2.8223786956631924,0.9942091784463614);
        \coordinate (W2) at (0.9881455681973705,2.748339302798502);
    
        \draw [shift={(2.7149165651566225,0)},] (0:0.2558385377085195) arc (0:83.83096092621358:0.2558385377085195);
        
        \draw [shift={(W1)},] (0:0.22) arc (0:83.8309609262136:0.22);
        \draw [shift={(W1)},] (83.8309609262136:0.2558385377085195) arc (83.8309609262136:167.66192185242716:0.2558385377085195);
        
        
        \draw [shift={(0,2.5948194798051945)},] (8.830960926213633:0.2558385377085195) arc (8.830960926213633:90:0.2558385377085195);
        \draw [shift={(0,2.5948194798051945)},] (8.830960926213633:0.20040685453834028) arc (8.830960926213633:90:0.20040685453834028);
        \draw [shift={(W2)},] (8.83096092621364:0.2558385377085195) arc (8.83096092621364:90:0.2558385377085195);
        \draw [shift={(W2)},] (8.83096092621364:0.20040685453834028) arc (8.83096092621364:90:0.20040685453834028);
        \draw [shift={(W2)},] (-72.33807814757273:0.21319878142376622) arc (-72.33807814757273:8.830960926213644:0.21319878142376622);
        \draw [shift={(W2)},] (-72.33807814757273:0.157767098253587) arc (-72.33807814757273:8.830960926213644:0.157767098253587);
        
        \draw [very thick] (0,4.5)-- (0,0);
        \draw [very thick] (5,0)-- (0,0);
        \draw [] (1,0) arc (0 : 90 : 1);
        \draw [] (0,1.5948194798051945) arc (-90 : 90 : 1);
        \draw [] (3.7149165651566225,0) arc (0 : 180 : 1);
        \draw [,dashed] (0.5257398542969663,0.8506454053269227)-- (0,0)
            node[pos=0.4,below right]{$r$};
        \draw [thick, blue] (0.9881455681973705,4.043597731705948)-- (W2);
        \draw [thick, blue] (W2)-- (V);
        \draw [thick, blue] (V)-- (W1);
        \draw [thick, blue] (W1)-- (4.430166711325904,0.9942091784463614);
        \draw [,dashed] (0,2.5948194798051945)-- (W2)
            node[pos=0.5, below]{$r$};
        \draw [,dashed] (W2)-- (1.560382488301416,2.837242915294451);
        \draw [,dashed] (2.7149165651566225,0)-- (W1)
            node[pos=0.5, left]{$r$};
        \draw [,dashed] (W1)-- (2.891073104860997,1.629750385478656);
        \draw [] (4.430166711325904,1)-- (4.430166711325904,0);
        \draw [] (1,4.043597731705948)-- (0,4.043597731705948);
        \draw [thick, blue,dashed] (1.2367685238557085,1.0588168446924053)-- (1.0328898481033684,0.8350560302118302);
        \draw [thick, blue] (1.2367685238557085,1.0588168446924053)-- (V);
        
        \draw [decorate , decoration={brace, mirror, amplitude=3pt},      
            xshift=0pt,yshift=-4pt]
        (0, 0) -- (2.7149165651566225,0) node [midway,yshift=-0.5cm] {$x$};
        \draw [decorate , decoration={brace, amplitude=3pt},      
            xshift=-4pt,yshift=0pt]
        (0, 0) -- (0,2.5948194798051945) node [midway,xshift=-0.5cm] {$y$};
        
        \def\nodesize{0.03}
        
        \fill [] (0,0) circle (\nodesize)
            node[below left]{$A_1$};
        \fill [] (0,4.5)
            node[above]{$A_3$};
        \fill [] (5,0)
            node[right]{$A_2$};
            
        \fill [blue] (W1) circle (\nodesize)
            node[black, below left]{$W_1$};
        \draw[shift={(W1)}] (0.15, 0.05)
            node[above right]{\large $\alpha$};
        \fill [] (2.7149165651566225,0) circle (\nodesize)
            node[below right]{$y(W_1)$};
            
            
        \fill [blue] (W2) circle (\nodesize)
            node[black, above left]{$W_2$};
        \draw[shift={(W2)}] (0.1, 0.15)
            node[above right]{\large $\beta$};
        \fill [] (0,2.5948194798051945) circle (\nodesize)
            node[above left]{$y(W_2)$};
            
            
        \fill [blue] (V) circle (\nodesize)
            node[black, above right]{$V$}
            node[black, left]{$120^\circ$};
        \draw[shift={(V)}] (0.1, -0.05) 
            node[below]{$120^\circ$};
            
        \fill [blue] (0.9881455681973705,4.043597731705948) circle (\nodesize)
            node[black, above]{$Z_2$};
        \fill [blue] (4.430166711325904,0.9942091784463614) circle (\nodesize)
            node[black, right]{$Z_2$};
        \fill [] (0,4.043597731705948) circle (\nodesize)
            node[left]{$C_{12}$};
        \fill [] (4.430166711325904,0) circle (\nodesize)
            node[below]{$C_{11}$};
        \fill [] (1.1,4.043597731705948)
            node[right]{$D_{12}$};
        \fill [] (4.430166711325904,1.1) 
            node[above]{$D_{11}$};;
    \end{tikzpicture}
   % \caption{Пересечение $\mathcal{C}$ с окрестностью угла}
    \label{minimizer90}
\end{figure}

==> ����������� (1)/pictures/PresentationStadion.tex <==
\begin{figure}[h]
    \centering
 

\begin{tikzpicture}[scale=1.1]

\foreach \y in {0, 3.51389977019889} {
    \draw[very thick, loosely dotted] 
        (-1, \y) -- (0, \y);
    \draw[very thick]
        (0, \y) -- (3.66, \y);
    \draw[very thick, loosely dotted] 
        (3.66, \y) -- (4.66, \y);
}
\draw[very thick] (-1, 0) arc (270:90:1.757);
\draw[very thick] (4.66, 0) arc (-90:90:1.757);


%\draw[thin, dashed] (0.2614137092297641 + 1, 0.0) arc (0:180:1);
%\draw[thin, dashed] (0.7842411276892922 + 1, 0.0) arc (0:180:1);
%\draw[thin, dashed] (1.3070685461488205 + 1, 0.0) arc (0:180:1);
\draw[thin, dashed] (1.8298959646083486 + 1, 0.0) arc (0:180:1);
%\draw[thin, dashed] (2.3527233830678767 + 1, 0.0) arc (0:180:1);
%\draw[thin, dashed] (2.875550801527405 + 1, 0.0) arc (0:180:1);
%\draw[thin, dashed] (3.398378219986933 + 1, 0.0) arc (0:180:1);
%\draw[thin, dashed] (1.8298959646083486 + 1, 3.75) arc (0:-180:1);


\draw[blue, thick] 
(0.0, 0.9652268503449002) -- 
(1.5684822553785844, 0.9652268503449002) --
(1.8298959646083486, 1.11615412573856) --
(2.0913096738381127, 0.9652268503449002) -- 
(3.659791929216697, 0.9652268503449002);

\node[blue] at (1.61,1.8) {$\Sigma_0$};

\draw[dashed] (0.0, 0.0) -- (0.0, 3.51389977019889);
\draw[dashed] (3.659791929216697, 0.0) -- (3.659791929216697, 3.51389977019889);

\fill[blue] (0.0, 0.9652268503449002) 
    circle (1.5pt) node[black, below right] {$A$};
\fill[blue] (3.659791929216697, 0.9652268503449002) 
    circle (1.5pt) node[black, below left] {$B$};

\draw[blue, thick] 
(1.8298959646083486, 1.11615412573856) -- 
(1.8298959646083486, 2.58208251632886);

\draw[thin, dashed] (1, 3.51389977019889) arc (0:-90:1);
\draw[thin, dashed] (2.66, 3.51389977019889) arc (180:270:1);

\draw[blue, thick]
(1.8298959646083486, 2.58208251632886) -- 
(0.9149479823041743, 3.11032798020668);

\draw[blue, thick] 
(1.8298959646083486, 2.58208251632886) -- 
(2.744843946912523, 3.11032798020668);



\end{tikzpicture}

\caption{A horseshoe is not optimal for long enough stadium if $R < 1.75r$.}
%КАЖЕТСЯ ЛИБО ЛОНГЭНАФ ЛИБО НЕРАВЕНСТВО. И НАВЕРНОЕ НЕ ДЛИННЫЙ А УЗКИЙ?
    \label{stadion}
\end{figure}
